Exploring the Impact of Training Data Distribution and Subword Tokenization on Gender Bias in Machine Translation

We study the effect of tokenization on gender bias in machine translation, an aspect that has been largely overlooked in previous works. Specifically, we focus on the interactions between the frequency of gendered profession names in training data, their representation in the subword tokenizer's vocabulary, and gender bias. We observe that female and non-stereotypical gender inflections of profession names (e.g., Spanish "doctora" for "female doctor") tend to be split into multiple subword tokens. Our results indicate that the imbalance of gender forms in the model's training corpus is a major factor contributing to gender bias and has a greater impact than subword splitting. We show that analyzing subword splits provides good estimates of gender-form imbalance in the training data and can be used even when the corpus is not publicly available. We also demonstrate that fine-tuning just the token embedding layer can decrease the gap in gender prediction accuracy between female and male forms without impairing the translation quality.

==> figures/fig_1D_pair_analysis_vertical.tex <==

\begin{figure}[!tb]
    \centering
    \begin{subfigure}{0.97\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/pairplot_de.pdf}
        \caption{German}
    \end{subfigure}
    \vfill
    \begin{subfigure}{0.97\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/pairplot_es.pdf}
        \caption{Spanish}
    \end{subfigure}
    \vfill
    \begin{subfigure}{0.97\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/pairplot_he.pdf}
        \caption{Hebrew}
    \end{subfigure}
    \caption{Pair analysis of gender prediction performance (F1), number of tokens, and the frequency of each profession in the OPUS-100 dataset. Each dot represents a profession in the male/female/pro-stereotypical/anti-stereotypical form. The diagonal plots show the density of the feature for the gender and stereotype sets.}
    \label{fig:1D}
\end{figure}

==> sections/X2_method_experiments.tex <==




We design a set of three experiments to evaluate our hypotheses about number of tokens and lexical translation accuracy and whether it has systematic effect on model's preference of words in specific gender.
\gabis{I wonder if it's better to separate some of this into a dedicated ``Research Questions'' section which formally defines what are our hypotheses, sthen this section can lay out the experiments to answer them. I'm not sure if it'll be too repetitive though.}

\subsection{Does a model prefer to generate words with less subwords?} 
\label{sec:1A}
\gabis{Is there a more succinct manner to write the research question? Given that we want to repeat it several times throughout the paper, this long phrasing is a bit cumbersome.}
We test lexical translation recall \barirep{in general domain}{over all words in the target language lexicl dictionary}. The evaluation procedure is as follows: 1.the translated texts are aligned with the source text on word level; 2. For each source word we check if it was translated to one of the correct translations from lexical dictionary (MUSE); 3. If the translation is correct we indicate target word as ``correctly predicted''; 4. If alignment does not contain correct translation, \barirep{each word paired with source language word in lexical dictionary is indicated}{the word is marked} as ``missed translation''. 

Finally, we compute \textit{generation recall} for each word in target dictionary as:

\begin{equation}
    \text{recall}_{lex} = \frac{correct_w}{correct_w + missed_w}
\end{equation}

We aggregate recall results for all words split into the same number of subword tokens by the target language tokenizer. Our expectation, is to see a decreasing recall for words split into more tokens.



\subsection{Are female and non-stereotypical forms split into more tokens?}
\label{sec:1B}
We analyze the human translations of profession names into female and male forms in German and Hebrew. We compare numbers of male and female words split into specific number of tokens by the target language tokenizer.

We expect that female forms will be split into more tokens than male forms, partially due to inflectional suffix appearing only in female forms. We also expect to observe a lower number of tokens for stereotypical forms (e.g. female ``nurse'', male ``mechanic'') than in anti-stereotypical ones, since the former group should be more present in the datasets used for training the tokenizer.

\subsection{Does a model prefer to translate profession word to a gender form with less tokens?}
\label{sec:1C}

We build upon two previous assumptions. We check the trend between difference of number of tokens for specific profession names and the accuracy of gender prediction in WinoMT test set.

We expect that the profession names with high difference in the number of tokens present in \barirep{female and male}{male and female} translation,i.e. the male form has more tokens than the female form, will be more prone to be translated into the shorter form (typically male one).

Finally, we conduct the analysis described in Section~\ref{sec:1A} for profession names. We want to compare  \textit{generation recall} of female and male forms that are split into the same number of tokens. If splitting is the main factor affecting accuracy of gender translation, the results for male and female profession should be close.


==> sections/X3_gedner_measures.tex <==
In some of our analysis we compute $\Delta G$, $\Delta S$ and $\Delta T$. 
$\Delta G$ is defined as the difference of male $F1$ score and female $F1$ score
where $F1$ score is the harmonic mean of recall and precision
For a profession p we mark the following notations:


$correct_{p,male}$ = number of times p was translated correctly as male.

$occurances_{p,male}$ = number of times p appeared as male in the dataset.

$translations_{p,male}$ = number of times p was translated as male


The male Recall and Precision of profession p is defined as
\begin{equation}
    \begin{array}{l}
    \text {Recall}_{p,male}
    =\frac{\text{correct}_{p,male}}{\text{occurances}_{p,male}} \\
    \\
    \text {Precision}_{p,male}
    =\frac{\text{correct}_{p,male}}{\text{translations}_{p,male}}
    \end{array}
\end{equation}

The female Recall and Precision are defined similarly.

And finally we get $\Delta G$ as follows
\begin{equation}
        \Delta G_p = \text{F1}_{p,male} - \text{F1}_{p,female}
\end{equation}

The greater $\Delta G$ is, better the model performed on the male profession compared to the female form.


$\Delta T$ for profession p is defined as the difference between the number of tokens for p in the male form and in the female form
\begin{equation}
    \Delta T_p = \text{Tokens}_{p,male} -\text{Tokens}_{p,female}
\end{equation}

$\Delta S$ is defined similarly to $\Delta G$ but with the difference of Pro and Anti stereotype professions.
$\Delta T$ in the context of $\Delta S$ is also referred to the difference in number of tokens of the Pro and Anti stereotype forms of the profession in the target language.

==> sections/X4_results.tex <==
\begin{figure*}[!tb]
    \begin{subfigure}{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/graph_1_mid_frequency_German.pdf}
        \caption{German}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/graph_1_mid_frequency_Hebrew.pdf}
        \caption{Hebrew}
    \end{subfigure}
    \caption{Lexical recall for words in general domain testset Tatoeba~\cite{tiedemann-2020-tatoeba}. The recalls were computed for unique words in target language. The height of each bar is the average recall of words split into specific number of tokens (subwords) shown on x-axis. For this plot we selected only words that were expected to appear system output between 10 and 100 times.
    \bari{we can see that the accuracy decreases when the number of tokens increase}}
    \label{fig:1A}
\end{figure*}


\subsection{\barirep{Are words split into less tokens easier to generate in target language?}{Does a model prefer to generate words with less tokens?}}
\label{sec:res-1A}

In Figure~\ref{fig:1A} we show the \textit{generation recall} for words in target language depending on the number of subwords they split into by the tokenizer. We observe significantly higher recalls for words that are not split into subwords (i.e. split into one token) for both German and Hebrew. This result supports assumption that words split into more subwords are less likely to be predicted in general domain. Importantly, SentencePiece \tomasz{SentecePiece} rely purely on training data, and is trained to keep frequently occuring sequences of bytes in one token, therfore frequent words tend not to be split into subwords. In order to marginalize the role of word frequency on generation accuracy, we present the results for unique words with medium frequency in the testing corpus (occuring between 10 to 100 times in the data). The results for most- and least-commmon words can be found in the appendix.





To answer this question, we asked native speakers to translate profession names from WinoMT to their languages (Hebrew and German). 

The Figures~\ref{fig:1B_3} and \ref{fig:1B_4} show how many translated profession names are split into specific number of sub-words. We observe that female forms tend to be split into more subwords than male ones. Only small portion of female forms is unsplitted in opposite to male ones \bari{in German 4 tokens words}. Similarly anti-stereotypical translations are split into less tokens than pro-stereotypical ones, howver the difference is smaller than in case of gender.
\bari{why does it hint to this conclusion?}
This result hints that female forms are split into more tokens because they appear less often in training corpora , but also because they consit of more characters \tomasz{More evidence needed here?}.

\begin{figure}[!tb]
    \centering
    \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/graph_3_de.pdf}
        \caption{German}
    \end{subfigure}
    \hfill
    \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/graph_3_he.pdf}
        \caption{Hebrew}
    \end{subfigure}
    \caption{Human translated profession names grouped by the number of subwords they were split in the target languages. On the x-axis: number of tokens per word (subwords). On th y-axis: the count of male and female forms professions in each of the groups. Male forms tend to be split into less subwords than female forms.}
    \label{fig:1B_3}
\end{figure}
\subsection{Are female words split into more tokens?}
\label{sec:res-1B}

\begin{figure*}[!tb]
    \begin{subfigure}{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/graph_4_de.pdf}
        \caption{German}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/graph_4_he.pdf}
        \caption{Hebrew}
    \end{subfigure}
    \caption{Human translated profession names grouped by the number of subwords they were split in the target languages. On the x-axis: number of tokens per word (subwords). On th y-axis: the count of pro- and anti-stereotypical forms professions in each of the groups. Pro-stereotypical forms tend to be split into less subwords than anti-stereotypical forms.}
    \label{fig:1B_4}
\end{figure*}



% \begin{figure*}[!tb]
%     \begin{subfigure}{0.45\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/graph_5_German_recall.pdf}
%         \caption{German}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.45\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/graph_5_Hebrew_recall.pdf}
%         \caption{Hebrew}
%     \end{subfigure}
%     \caption{Figures from 1C Recall against Delta T}
%     \label{fig:1C_recall}
% \end{figure*}

\begin{figure}[!tb]
    \centering
    \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/graph_5_German_delta_g.pdf}
        \caption{German}
    \end{subfigure}
    \hfill
    \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/graph_5_Hebrew_delta_g.pdf}
        \caption{Hebrew}
    \end{subfigure}
    \caption{$\Delta G$ as difference between F1-score for male and female test instances for each of paired translations. $\Delta T$ is the difference between number of subwords in a male and a female form. We observe negative correlation between two measures ($\rho=-0.11$ for Hebrew and $\rho=-0.25$ for German).}
    \label{fig:1C_delta_g}
\end{figure}


\begin{figure}[!tb]
    \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/graph_5_German_delta_s.pdf}
        \caption{German}
    \end{subfigure}
    \hfill
    \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/graph_5_Hebrew_delta_s.pdf}
        \caption{Hebrew}
    \end{subfigure}
    \caption{$\Delta S$ as difference between F1-score for pro- and anti-stereotypical test instances for each of paired translations. $\Delta T$ is the difference between number of subwords in a pro- and a anti-stereotypical translation. We observe negative correlation between two measures ($\rho=-0.41$ for Hebrew and $\rho=-0.37$ for German).}
    \label{fig:1C_delta_s}
\end{figure}


% \begin{figure*}[!tb]
%     \begin{subfigure}{0.49\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/graph_6_per_gender_German.pdf}
%         \caption{German}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.49\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/graph_6_per_gender_Hebrew.pdf}
%         \caption{Hebrew}
%     \end{subfigure}
%     \label{fig:1C_lex_recall_gender}
%     \caption{Lexical recall for profession in WinoMT \cite{stanovsky-etal-2019-evaluating}. The recall is averaged for target language words in the same gender split into the same number of tokens (subwords) shown on x-axis. Female forms tend to have lower recall than male ones even when they consit of the same number of subwords.}
% \end{figure*}



% \begin{figure*}[!tb]
%     \begin{subfigure}{0.49\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/graph_6_per_streotype_German.pdf}
%         \caption{German}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.49\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/graph_6_per_streotype_Hebrew.pdf}
%         \caption{Hebrew}
%     \end{subfigure}
%     \label{fig:1C_lex_recall_stereotype}
%     \caption{Lexical recall for profession in WinoMT \cite{stanovsky-etal-2019-evaluating}. The recall is averaged for target language translations with the same sterotypy (pro or against) split into the same number of tokens (subwords) shown on x-axis.}
% \end{figure*}

\subsection{Does difference in number of tokens affect preference of specific form in translation?}
\label{sec:res-1C}

We compute the standard gender bias measures from \citet{stanovsky-etal-2019-evaluating} for pairs of translations obtained from human annotation process. Afterwards we compare them with the difference in number of subwords in two translation forms (male, female or pro-, anti-stereotypical) called $\Delta T$. The results are presented in Figures~\ref{fig:1C_delt_g, fig:1C_delta_s}. We observe negative correlations between $\Delta T$ and both $\Delta G$ and $\Delta S$. The relationship is stronger in the latter case. This finding supports our hypothesis that diverging number of tokens leads to model's preference toward a form with less tokens (typically male or stereotypical one as shown in Section~\ref{sec:res-1B}.

Moreover for translation pairs with $\Delta T=0$ mean and median of bias measure distribution is close to zero (with the exception of $\Delta G$ for Hebrew). Therefore, we infere that model's translation is less skewed when the choice is between target language forms with the same numbers of subwords.

% In the next step we conducted lexical recall evaluation for male and female professions (Figure~\ref{fig:1C_lex_recall_gender}). The results were less encouraging, we observed that for profession words unsplit in target language recall is higher for male than female forms. The difference decrease for forms split into more tokens. Similarly pro-stereotypical translations tended to achieve higher lexical recall than anti-stereotypical ones as shown on Figure~\ref{fig:1C_lex_recall_stereotype}. Notable exception are unsplit translation to German, where anti-stereotypical forms achieved higher average recall. 

% It is important to note that in case of recall analysis, we averaged results for multiple professions' translation and for instance unsplitted female forms could appear in harder to translate contexts than unsplitted male forms. Morover, the number of professions belonging to each analyzed been can significantly vary.

==> sections/X6_discussion.tex <==

Our results show that tokenization plays a role in the accuracy of gender translation.

However, we still see some bias towards male professions in Figures~\ref{fig:1C_delta_g}~and~\ref{fig:1C_delta_s} where the median (orange line) of bias measures is above 0 in cases where $\Delta T=0$. We also observe a high variance of \barirep{their}{the male ande female forms} distributions. Therefore, we conclude that tokenization is not the only factor causing this tendency.

In fact, our analysis of sample of model's training corpora showed that \barirep{subword splitting is only proxy factor [idk if it's the best name] correlated with gender form's frequency in the training corpus.}{Gender Bias is independant of number of tokens, and their relationship is confounded by the frequency.} Frequency has a more significant influence on preferred gender form in translation. 
\tomasz{maybe add this to the conclusions.}{moved to conclusion}

Our findings indicate the causal relation shown in Figure~\ref{fig:shwartz}.
Namely, we find that while it may initially seem that the number of subword tokens may explain the translation accuracy of a given word, they are, in fact, independent of one another given the frequency of the word in the training set.


% \tomasz{Following is not applicable anymore}
% We assume that the other factors are based on the dataset that the translation model learned from, which might contain more male form professions rather than the female form. For example, in Hebrew, when the gender of the person is unknown, it is treated as male by default.



% The bias can also be affected by the dataset that the tokenizer was trained on. Words that are less frequent in this dataset will be split into more tokens.
% An example of frequencies analysis of training dataset was introduced by \citet{DBLP:journals/corr/abs-2109-03858}. They created a pronoun distribution histogram of BUG dataset, which contains the pronouns ``his'', ``her'', ``himself'', ``herself'', ``she'' and ``he''. They show that every male pronoun is more frequent in the dataset than the female pronoun, and in total, there are
% 82K (76\%) masculine pronouns and 26K (24\%) feminine pronouns.
% In addition, we analyzed the Wikipedia dataset in Opus and found out that male form professions appear twice as often as female forms.



\subsection{Future Work}
% \barirep{In future work,  we will focus on extending the analysis to more translation systems e.g. BART \cite{tang2020multilingual}, Facebook NMT \cite{fan2020beyond}, which utilize  other subword tokenization algorithms. Furthermore, we want to apply our findings in the practical debiasing technique, where we would add professions names to the target tokenizer vocabulary to protect them from splitting into subwords.
% We will also focus on mapping more factors for the bias, such as training dataset distributions of gendered forms.


In future work, we will focus on mapping more factors for the bias by isolating more features like model structure, the order of the examples in the training process and more. We will examine the dependencies of tokens, frequency, and gender bias on a larger scale, with more words, and test the hypotheses on a complete different type of tokenization such as character level tokenization.



% \begin{itemize}
%     \item Compare number of tokens with word's frequency in training corpora (or similar)
%     \item Generalize the analysis for another translation system preferably with a different tokenizer, e.g. BART, Facebook m2m
%     \item Apply the findings to debising, e.g. adding all female anti-stereotypical forms to the vocabulary.
% \end{itemize}

==> sections/XX2_methodology.tex <==
We analyze the OpusMT translation model \cite{TiedemannThottingal:EAMT2020} and \textsc{mBART50} \cite{tang2020multilingual} from English to German and Hebrew.\footnote{The results for \textsc{mBART} are presented in Appendix~\ref{}} \gabis{Why those specific models and languages?} \gabis{Why are we presenting results in an appendix?}

% \bari{We analyse the performance of those models with respect of number of tokens and frequency of the training dataset.}

% \subsection{Measures of Gender Bias}
\tomasz{IMO we need to further reduce the discussion about $\Delta G$ and $\Delta S$ and clearly say that F1 (and other measures) are computed per profession. Then hint the reader to the appendix... }

To measure gender bias, we use two metrics employed by \citet{stanovsky-etal-2019-evaluating}: $\Delta G$ measure the difference in translation accuracy between masculine and feminine entities,  while $\Delta S$ measures the difference between pro-stereotypical (e.g., male secrateries) \david{male secretaries are IMO anti-stereotypical} and anti-stereotypical instances (e.g., female doctors) gender role assignemnts.\footnote{We use previous works definitions for what constitutes a stereoypical assignemnt~\citep{.}
% The greater $\Delta G$ is, the better the model performed for the masculine forms compared to the feminine ones, and the same concept applies for $\Delta S$.
% The Pro and Anti stereotype professions used for $\Delta S$ same list of WinoBias professions separated to male and female stereotypes by \citet{zhao-etal-2018-gender}. For example, the male form of manager and the female form of nurse are pro stereotype, and the male form of receptionist and female form of driver are anti stereotype.


We define our measure $\Delta T$ for profession $p$ as the difference between the number of tokens for $p$ in the male and female forms in the context of $\Delta G$, and the difference in number of tokens of the Pro and Anti stereotype forms in the context of $\Delta S$. 
Both computed on words in target language.

 (An explanation about what $F1$ scores means in gender context can be found in the Appendix \ref{f1_gender}).  
% \begin{equation}
%     \Delta T_p = \text{Tokens}_{p,male} -\text{Tokens}_{p,female}
% \end{equation}




